Machine Learning: The Basics

Machine learning (ML) has become a commodity in our every-day lives. We routinely ask ML empowered smartphones to suggest lovely food places or to guide us through a strange place. ML methods have also become standard tools in many fields of science and engineering. A plethora of ML applications transform human lives at unprecedented pace and scale. This book portrays ML as the combination of three basic components: data, model and loss. ML methods combine these three components within computationally efficient implementations of the basic scientific principle "trial and error". This principle consists of the continuous adaptation of a hypothesis about a phenomenon that generates data. ML methods use a hypothesis to compute predictions for future events. We believe that thinking about ML as combinations of three components given by data, model, and loss helps to navigate the steadily growing offer for ready-to-use ML methods. Our three-component picture of ML allows a unified treatment of a wide range of concepts and techniques which seem quite unrelated at first sight. The regularization effect of early stopping in iterative methods is due to the shrinking of the effective hypothesis space. Privacy-preserving ML is obtained by particular choices for the features of data points. Explainable ML methods are characterized by particular choices for the hypothesis space. To make good use of ML tools it is instrumental to understand its underlying principles at different levels of detail. On a lower level, this tutorial helps ML engineers to choose suitable methods for the application at hand. The book also offers a higher-level view on the implementation of ML methods which is typically required to manage a team of ML engineers and data scientists.

==> AI18_macros.tex <==
%\newcommand{\Tt}[0]{\boldsymbol{\theta}}
%\newcommand{\XX}[0]{{\cal X}}
%\newcommand{\ZZ}[0]{{\cal Z}}
%\newcommand{\vx}[0]{{\bf x}}
%\newcommand{\vv}[0]{{\bf v}}
%\newcommand{\vu}[0]{{\bf u}}
%\newcommand{\vs}[0]{{\bf s}}
%\newcommand{\vm}[0]{{\bf m}}
%\newcommand{\mX}[0]{{\bf X}}
%\newcommand{\vw}[0]{{\bf w}}
%\newcommand{\D}[0]{{\mathcal{D}}}
%\newcommand{\mP}{\mathbf{P}}
%\newcommand{\E}[0]{{\mathbb{E}}}
%\newcommand{\vy}[0]{{\bf y}}
%\newcommand{\vb}[0]{{\bf b}}
%\newcommand{\vr}[0]{{\bf r}}
%\newcommand{\vz}[0]{{\bf z}}
%\newcommand{\N}[0]{{\mathcal{N}}}
%\newcommand{\vc}[0]{{\bf c}}
%\newcommand{\norm}[1]{\Vert  {#1} \Vert}
%%\newcommand{\XX}[0]{X}
%%\newcommand{\ZZ}[0]{Z}
%\newcommand{\bmx}[0]{\begin{bmatrix}}
%\newcommand{\emx}[0]{\end{bmatrix}}
%%\newcommand{\norm}[1]{\lVert#1\rVert}
%\newcommand{\T}[0]{\text{T}}
%\DeclareMathOperator*{\rank}{rank}
%\newcommand\defeq{:=}
%\newcommand\eigvecS{\hat{\mathbf{u}}} 
%\newcommand\eigvecCov{\mathbf{u}} 
%\newcommand{\featuredim}{d}
%\newcommand{\samplesize}{N}
%\newcommand{\sampleidx}{i} 
%\newcommand{\target}{y}
\newcommand{\state}{s} 
\newcommand{\statespace}{\mathcal{S}} 
\newcommand{\timeidx}{t} 
\newcommand{\optpolicy}{\pi_{*}} 
\newcommand{\appoptpolicy}{\hat{\pi}} 
\newcommand{\dummyidx}{j} 
\newcommand{\gridsizex}{K}
\newcommand{\gridsizey}{L}
%\newcommand{\error}{E}
\newcommand{\reward}{R}
\newcommand{\cumreward}{G}
\newcommand{\return}{\cumreward}
\newcommand{\action}{a}
\newcommand\actionset{\mathcal{A}}
%\newcommand\dataset{\mathbb{X}}
%\newcommand{\inspace}{\mathcal{X}}
%\newcommand{\sigmoid}{\sigma}
\newcommand{\obstacles}{\mathcal{B}}
%\newcommand{\outspace}{\mathcal{Y}}
%\newcommand{\hypospace}{\mathcal{H}}
%\newcommand{\emperror}{\mathcal{E}}
%\newcommand{\generror}{\mathcal{E}}
%\DeclareMathOperator{\supp}{supp}
%\newcommand{\loss}[3]{L({#1},{#2},{#3})} 
%\newcommand{\loss}[2]{L({#1},{#2})} 
%\newcommand{\determinant}[1]{{\rm det}({#1})} 
%\newcommand{\prob}[1]{P({#1})} 
%\newcommand{\pdf}[1]{p({#1})} 
%\def \expect {\mathbb{E} }
%\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\valuefunc}[1]{v_{#1}}
\newcommand{\gridcell}[2]{\langle #1, #2 \rangle}
\newcommand{\pair}[2]{\langle #1, #2 \rangle}
\newcommand{\mdp}[5]{\langle #1, #2, #3, #4, #5 \rangle}
\newcommand{\actionvalue}[1]{q_{#1}}
\newcommand{\transition}{\mathcal{T}}
\newcommand{\policy}{\pi}
\newcommand{\charger}{c}
\newcommand{\itervar}{k}
\newcommand{\discount}{\gamma}
\newcommand{\rumba}{Rumba}
\newcommand{\actionnorth}{\rm N} 
\newcommand{\actionsouth}{\rm S} 
\newcommand{\actioneast}{\rm E} 
\newcommand{\actionwest}{\rm W}
\newcommand{\chargingstations}{\mathcal{C}}
%\def \prob {{\rm P} }




==> EdgesKarate.tex <==
a,b
2,1
3,1 
3,2
4,1 
4,2 
4,3
5,1
6,1
7,1 
7,5 
7,6
8,1 
8,2 
8,3 
8,4
9,1 
9,3
10,3
11,1 
11,5 
11,6
12,1
13,1 
13,4
14,1 
14,2 
14,3 
14,4
17,6 
17,7
18,1 
18,2
20,1 
20,2
22,1 
22,2
26,24 
26,25
28,3 
28,24 
28,25
29,3
30,24 
30,27
31,2
31,9
32,1 
32,25 
32,26 
32,29
33,3 
33,9 
33,15 
33,16 
33,19 
33,21 
33,23 
33,24 
33,30 
33,31 
33,32
34,9
34,10
34,14 
34,15 
34,16 
34,19 
34,20 
34,21 
34,23 
34,24 
34,27
34,28 
34,29 
34,30 
34,31 
34,32 
34,33

==> NodesKarate.tex <==
nodeID,a,b
1,0.64,1.90
2,-0.06,2.15
3,1.98,2.44
4,-2.8,2.13
5,4.12,1.38
6,-0.32,1.50
7,2.22,1.38
8,-3.72,2.28
9,1.2,2.65
10,-1.02,2.96
11,1,1.43
12,6.86,1.41
13,-3.66,1.80
14,-0.8,2.43
15,3.26,3.20
16,1.62,3.15
17,-1.4,1.56
18,3.2,1.63
19,8.54,3.11
20,4.24,2.12
21,10.3,2.70
22,-4.06,1.98
23,10.2,2.97
24,10.1,2.81
25,13.26,2.43
26,13.3,2.29
27,4.96,3.22
28,8.86,2.47
29,8.18,2.27
30,7.06,3.17
31,3.04,2.63
32,11.84,2.61
33,6.26,2.89
34,5.54,2.77

